PCB-ready breakout boards: Bridging the gap between electronics prototyping and production

Electronics prototyping using breakout boards allows designers with and without an engineering background to rapidly create interactive prototypes. However, when it comes to transition to a production-ready PCB design, stagnation exists due to the high skill floor required for PCB design. While PCB design automation has been used successfully in recent research tools to reduce the required expertise, little has been done to integrate these tools directly into the electronics prototyping cycle. This position paper aims to bring attention to the possibility of integrating recent PCB design automation paradigms into the electronics prototyping cycle for the creation of PCB-ready breakout boards: breakout boards whose designs would have the ability to be pipelined directly into new user interfaces that leverage the use of automation for the rapid creation of production-ready PCB designs.

==> Limitations.tex <==
%auto-ignore
\section{Limitations and Future Work}
\label{sec:limitations}


==> challenges.tex <==
\section{Design Challenges}
\label{sec:challenges}


==> intro.tex <==
%auto-ignore
\section{IntrodUction}
\label{sec:introdUction}

Prototyping using breakout boards is one of the three most popular paradigms when it comes to prototyping with electronic components (cite). Breakout boards consist of a set of modular PCBs, each containing multiple electronic components, which can be easily interconnected using breadboards for interactive design exploration or circuit debugging. Anyone can design and distribute breakout boards without affecting the compatibility between them, popular distributors include Arduino, Sparkfun, and Adafruit (cite).

After electronics prototyping, designers transfer the physical connections made between the breakout boards into a virtual representation format known as electronic schematic. Electronic schematics provide the designer with a simpler visual interactive format for connecting electronic components, where even dimensional blocks are used instead of irregular electronic component footprint shapes. After drawing the schematics, designers generate the PCB layout drawing virtual copper lines traces between electronic components footprints. After generating the schematic and PCB layout of the circuit, the circuit is considered ready for manufacturing. Popular PCB design tools include KiCad, Altium, Fusion 360.

Through the teaching of various classes where students with no prior electronics experience are taught circuit design, we have observed that one of the main problems students have is translating electronic prototypes to a PCB design, a design with a smaller and more rigid form factor, after the prototyping stage is complete. PCB design which is often the main goal after electronics prototyping.  We identify this problem caused by the following reasons: (1) The steep learning curve required to use PCB design tools (e.g.,Altium, Fusion 360, KiCad), (2) Understanding each of the components on the breakout boards and separating those required for the final design.

Commercial tools such as Sparkfun's À La Carte (ALC)~\cite{SparkfunALC} and Altium's Upverter Modular~\cite{AltiumUpverterModular} have taken small steps to improve this situation. These tools allow designers to choose different breakout boards or pre-tested circuit blocks, and allow their integration to create complete PCB designs. However these tools are non-automated, and require one or more engineers to manually create the full schematic and PCB design. A process with a design fee that can approach \$1,000 per design~\cite{SparkfunALCFaq}. 


Lambrichts et al. [22] 

Interactive electronic schematic design has been established as a de facto process that precedes PCB layout design. In this interactive design, users draw schematics by placing virtual electronic component symbols on virtual sheets and connect their signals together, a model used in many popular schematic capture tools (e.g., KiCad, Altium, Fusion 360). The falling cost of circuit board manufacturing processes has made hardware design more accessible than ever before, opening up professional-quality circuit design to students, hobbyists, and others but making the weaknesses of schematic capture tools more evident.

The growing community of circuit designers has noted that one of the biggest problems with schematic capture tools is the process of reusing and merging schematic blocks~\cite{lin2019beyond}. While some current circuit design tools provide some forms of schematic reuse, these mechanisms do not provide information about the capabilities of the blocks, for example, signal types, required voltages, among others. This makes composing reusable blocks to build new designs fraught with design challenges. Design challenges that constantly lead to connection errors and require designers to carefully analyze each schematic block they wish to combine, making schematic block reuse a less popular option among circuit designers.

Commercial block-based circuit design tools such as Sparkfun's À La Carte (ALC)~\cite{SparkfunALC} and Altium's Upverter Modular~\cite{AltiumUpverterModular} have taken small steps to improve this situation. These tools allow designers to choose different pre-tested circuit blocks, such as  microcontrollers, sensors, and connectors, and allow their integration to create complete new designs. Yet, although these tools have novel interactive design flows, the processes for merging schematic blocks still requires one or more engineers to manually create the full schematic as well as to check for any connection errors, an engineering design fee that can approach \$1,000 per design~\cite{SparkfunALCFaq}. 
% Furthermore, these tools are limited to a fixed number of schematic blocks that can be used, making the tools unscalable by the designer community. 

While popular opinions deny the need for better reuse processes~\cite{AltiumDeviceSheet}, the rise and interest in tools that can simplify the reuse process for schematics blocks suggests otherwise. Comparing the current state of reuse capabilities in schematic design with software design would be equivalent to software designers figuring out which data types (e.g., bool, int, char) are needed as input parameters and return values for each function by reading its code. In addition to understanding the input and output data types required by functions, data type information in software makes possible the detection of common data type errors at compile or real time, also known as type checking, a form of constraint validation. In schematics, the analog for software's data types are electrical interfaces that specify the compatible voltages, electrical currents, and data transfer interfaces (e.g., Serial, I2C, or PCIe).  These interface types, if properly encoded, can provide "type" checking for hardware designs~\cite{garza2019amalgam,AltiumUpverterModular,garza2021appliancizer}.

Although recent work ~\cite{lin2020polymorphic,jitpcb} has explored the addition of type information as well as the use of constraint validation mechanisms of connections for building circuits by proposing the use of board-level hardware description languages (HDLs). These tools are code-oriented and decoupled from the traditional visual and interactive schematic and circuit design flow, requiring circuit designers to learn programming languages. A learning task that requires a steep learning curve for novices or beginners without the help of visual and interactive interfaces. In addition, the use of code-based schematic model representations makes it impossible to reuse existing schematic designs. To date, there is no visual interactive tool that integrates the benefits of adding type information to schematic blocks, as well as implements error detection mechanisms in the merge process.

% In the hardware side, the use of hardware protocol interfaces (eg, I2C, SPI, GPIO) to transmit information between integrated circuits (ICs) have been considered as standardized data like types for schematic blocks by multiple tools.

% ~\jorge{remove?}Efficient reuse of circuit blocks is an important part of designing more complex systems. In programming the reuse of instructions in the form of functions, objects, or software packages are the backbone of modern programming, allowing programmers to build more elaborate systems that would take months or years otherwise. One of the reuse methods used in programming is the use of data types, where bytes go from being a set of empty arrays of bits to something with properties, capabilities, and restrictions (e.g., boolean, int, float, char). Functions and objects leverage the use of standard data types as I/O parameters for code blocks to be reused efficiently by the programmers community. As example, If a function block requires a boolean parameter, by restriction, it can only be connected to other blocks of code by the same data type. This reuse model is very efficient, however, is inexistent in schematic captures as there are no standards that define which signals or set of signals have what properties or characteristics, therefore making circuit designer unable to easily understand the circuit blocks to reuse in modern schematic capture tools.

In this paper, we address these shortcomings with \emph{TypedSchematics}, an interactive design tool that allows designers to annotate existing schematic blocks with type information enabling real-time detection of connection errors. To detect connection errors, TypedSchematics implements a similar approach to type checking using hardware protocol interfaces as a base which we call \emph{\interfacecheking{}}. A method that makes schematic blocks reuse and the merging process safer and faster. 


Compared to board-level HDLs, TypedSchematics leverages the already established traditional design flow for easier adoption. An expressive syntax facilitates annotating schematic blocks with type information for easier integration into our interactive tool.

In contrast to existing commercial solutions, such as Sparkfun ALC and Altium Upverter, which require external engineers to integrate or merge schematic design blocks, our typed syntax makes possible the automation of the merging step, allowing the rapid and automatic generation of full schematic designs.

In creating TypedSchematics, we noticed that in the process of merging schematic blocks, connecting power signals (e.g., Ground, VDD) becomes a repetitive task, as well as causing a pile up of wires or tags, producing a less clear design layout.

To create a clearer layout, TypedSchematics also introduces \textit{"Mats"}, a new visual schematic representation model for schematic blocks that uses a combination of tree and graph structures. This new approach allows breaking down the traditional structure consisting of a single schematic graph into one that is more efficient for schematic blocks, eliminating unnecessary signal connections and reducing interaction costs.

A data flow programming paradigm is also seamlessly integrated with the visual schematic representation model for running \interfacecheking{} on block connections.


Overall, the contributions of our work are as follows:
\begin{itemize}
    \item A method of adding type information to existing schematic blocks that enables real-time detection of connection errors, facilitating the process of merging schematic blocks using interactive designs.
    \item The introduction of Mats, a schematic representation model for schematic blocks that reduces design interaction costs.
\end{itemize}

The rest of this paper is organized as follows. \refsec{sec:related} describes previous work and techniques for reusing schematic designs and discusses existing block-based interfaces for circuit design. \refsec{sec:challenges} explains some of the design challenges with schematic blocks.
\refsec{sec:overview} introduces TypedSchematics. 
\refsec{sec:examples} demonstrates our tool capabilities by describing two devices made with TypedSchematics.
\refsec{sec:userstudy} and \refsec{sec:results} demonstrates how TypedSchematics addresses the design challenges with a user study, and \refsec{sec:conclude} concludes.

% \footnote{footnote}



==> related.tex <==
%auto-ignore
\section{Related Work}
\label{sec:related}

In this section we discuss previous work relevant to this discussion. 

\subsection{Non-automated user interfaces for fast production-ready PCB designs.}

Commercial tools such as Sparkfun's À La Carte (ALC)~\cite{SparkfunALC} and Altium's Upverter Modular~\cite{AltiumUpverterModular} have taken small steps to bridge the gap between prototype and production. These tools allow designers to choose different breakout boards, development boards or pre-tested circuit blocks, and allow their integration to create complete PCB designs. However these tools are non-automated, and require one or more engineers to manually create the full schematic and PCB layout design. A process with a design fee that can approach \$1,000 per design~\cite{SparkfunALCFaq}. In addition, having no standards for scaling the number of modules that can be used prevents community collaboration, limiting the designs that can be achieved with these tools.

\subsection{PCB design automation tools}


Several research tools have explored new circuit design approaches that take advantage of automation to rapidly create schematic and PCB layout designs. Echidna[], Appliancizer[], Polymorphic Blocks[] are examples of tools that take advantage of automation to explore new design paradigms that increase the abstraction of circuit design, making PCB design easier. Echidna enables the automatic generation of ready-to-manufacturer PCBs from virtual modular schematic designs. In Echidna, the design is abstract to the selection of components to be used and the software generates a complete PCB layout output. Appliancizer~\cite{garza2021appliancizer}, goes further, abstracting the design to the GUI level, allowing automated PCB layout, firmware, and interface simulation generation from web interfaces. Polymorphic Blocks~\cite{} takes a different direction by allowing automated generation of schematic designs from hardware description languages.


==> results.tex <==
%auto-ignore
\section{Results}
\label{sec:results}


==> userstudy.tex <==
%auto-ignore
\section{User Study}
\label{sec:userstudy}
